Two-Timescale Joint Precoding Design and RIS Optimization for User Tracking in Near-Field MIMO Systems

In this paper, we propose a novel framework that aims to jointly design the reflection coefficients of multiple RISs and the precoding strategy of a single BS to optimize the self-tracking of the position and the velocity of a single multi-antenna UE that moves either in the far- or near-field region. Differently from the literature, and to keep the overall complexity affordable, we assume that RIS optimization is performed less frequently than localization and precoding adaptation. The proposed procedure leads to minimize the inverse of the received power in the UE position uncertainty area between two subsequent optimization steps. The optimal RIS and precoder strategy are compared with the classical beam-focusing strategy and with a scheme that maximizes the communication rate. It is shown that if the RISs are optimized for communications, their configuration is suboptimal when used for tracking purposes. Numerical results show that in typical indoor environments with only one BS and a few RISs operating on millimeter waves, high location accuracy in the range of less than half a meter can be achieved.

==> def_LIS.tex <==
\newcommand{\rednote}[1] {{\color{red}$\blacktriangleright${#1}$\blacktriangleleft$}}
\newcommand{\blue}[1] {{\color{blue}{#1}}}
\newcommand{\virg}[1] {``{{#1}}''}




%---------------------%
%       References    %
%---------------------%
\newcommand{\fig}[1]{Fig.~\ref{#1}}
\newcommand{\sect}[1]{Sec.~\ref{#1}}
\newcommand{\apd}[1]{Appendix~\ref{#1}}
\newcommand{\eq}[1]{(\ref{#1})}

%


% Symbols definitions

\newcommand{\Real}[1]{\Re \left \{ #1\right \}}
\newcommand{\en} {E}
\newcommand{\td}[1] {\tilde{#1}}
\newcommand{\lt}[1] {{\td{\lambda}}_{#1}}
\newcommand{\bl}[1] {\text{\boldmath ${\lambda}$}_{#1}}
\newcommand{\blt}[1] {\text{\boldmath $\td{\lambda}$}_{#1}}
\newcommand{\vg}[1] {{\mbox{{\boldmath ${#1}$}}}}
\newcommand{\vgs}[2] {\vg{#1}_{#2}}

\newcommand{\PX}[1] {{\mathbb{P}}\left\{{#1}\right\}}
\newcommand{\EX}[1] {{\mathbb{E}}\left\{{#1}\right\}}
\newcommand{\EXs}[2] {{\mathbb{E}}_{{#1}}\!\!\left\{{#2}\right\}}
\newcommand{\Var}[1] {{\text{Var}}\left ({#1}\right )}

\newcommand{\CN}[1]{{\mathcal{CN}} \left (0, #1\right )}

\newcommand{\pX}[1] {{\mathbf{p}}\left\{{#1}\right\}}


\newcommand{\Hone} {\mathcal{H}_1}
\newcommand{\Hzero}{\mathcal{H}_0}
\newcommand{\hatHone} {\hat{\mathcal{H}}_1}
\newcommand{\hatHzero}{\hat{\mathcal{H}}_0}

\newcommand{\Mu} {\mathcal{M}_u}
\newcommand{\Mc}{\mathcal{M}_c}

\newcommand{\boldA} {{\bf{A}}}
\newcommand{\boldg} {{\bf{g}}}
\newcommand{\bolds} {{\bf{s}}}
\newcommand{\boldf} {{\bf{f}}}
\newcommand{\bolda} {{\bf{a}}}
\newcommand{\boldp} {{\bf{p}}}
\newcommand{\boldk} {{\bf{k}}}
\newcommand{\boldK} {{\bf{K}}}
\newcommand{\boldu} {{\bf{u}}}
\newcommand{\boldc} {{\bf{c}}}
\newcommand{\boldV} {{\bf{V}}}
\newcommand{\boldX} {{\bf{X}}}
\newcommand{\boldY} {{\bf{Y}}}
\newcommand{\boldW} {{\bf{W}}}
\newcommand{\boldE} {{\bf{E}}}
\newcommand{\boldJ} {{\bf{J}}}

\newcommand{\boldm} {{\bf{m}}}
\newcommand{\boldP} {{\bf{P}}}
\newcommand{\boldF} {{\bf{F}}}
\newcommand{\boldG} {{\bf{G}}}
\newcommand{\boldR} {{\bf{R}}}
\newcommand{\boldC} {{\bf{C}}}

%\newcommand{\boldT} {{\bf{T}}}
%\newcommand{\boldF} {\bf{F}}
\newcommand{\boldI} {{\bf{I}}}

\newcommand{\meanr} {{\overline{r}}}
\newcommand{\meanboldr} {{\overline{\bf{r}}}}
\newcommand{\boldn} {{\bf{n}}}
\newcommand{\boldx} {{\bf{x}}}
\newcommand{\boldy} {{\bf{y}}}
\newcommand{\boldh} {{\bf{h}}}

\newcommand{\boldv} {{\bf{v}}}
\newcommand{\boldt} {{\bf{t}}}
\newcommand{\meanw} {{\overline{w}}}
\newcommand{\meanboldw} {{\overline{\bf{w}}}}
\newcommand{\boldd} {{\bf{d}}}
\newcommand{\boldalpha} {\bf{\alpha}}
\newcommand{\boldbeta} {\bf{\beta}}
\newcommand{\boldgamma} {\bf{\gamma}}
\newcommand{\boldrho} {\bf{\rho}}
\newcommand{\boldhc} {\bf{h}_{\text{c}}}

\newcommand{\Pd} {P_{\text{d}}}
%\newcommand{\Pf} {P_{\text{f}}}

\newcommand{\Pb} {P_{\text{b}}}

\newcommand{\Rb} {R_{\text{b}}}
\newcommand{\Ep} {E_{\text{p}}}


\newcommand{\Ew} {E_{\text{w}}}
\newcommand{\Eref} {E_{\text{ref}}}
\newcommand{\Gref} {G_{\text{ref}}}
\newcommand{\Tp} {T_{\text{p}}}
\newcommand{\Td} {T_{\text{d}}}

\newcommand{\ts} {t_{\text{s}}}
\newcommand{\Ta} {T_{\text{a}}}


\newcommand{\Nps} {N_{\text{ps}}}
\newcommand{\tp} {\tau_{\text{p}}}
\newcommand{\Es} {E_{\text{s}}}
\newcommand{\Eb} {E_{\text{b}}}
\newcommand{\Ts} {T_{\text{s}}}
\newcommand{\Tf} {T_{\text{f}}}
\newcommand{\Tc} {T_{\text{c}}}
\newcommand{\Th} {T_{\text{h}}}
\newcommand{\Tb} {T_{\text{b}}}
\newcommand{\Tob} {T_{\text{ob}}}

\newcommand{\Na} {N_{\text{A}}}

\newcommand{\Nsym} {N_{\text{sym}}}
\newcommand{\tint} {T_{\text{int}}}
\newcommand{\TX}[1] {{\mathbb{T}}\left [{#1}\right ]}
\newcommand{\Prob}[1] {\text{P}\left\{{#1}\right\}}

\newcommand{\Nch} {N_{\text{ch}}}
\newcommand{\Lp} {L_{\text{p}}}
\newcommand{\dref} {d_{\text{ref}}}
\newcommand{\wref} {w_{\text{ref}}}
\newcommand{\Wref} {W_{\text{ref}}}
\newcommand{\Href} {H_{\text{ref}}}
\newcommand{\ZA} {Z_{\text{A}}}
\newcommand{\taup} {\tau_{\text{f}}}
%\newcommand{\etaup} {\hat{\tau}_{\text{f}}}
\newcommand{\taud} {{\tau_{\text{d}}}}
\newcommand{\etaud} {\hat{\tau}_{\text{d}}}
\newcommand{\toa} {\tau}
\newcommand{\etoa} {\hat{\tau}}
\newcommand{\Beff} {B_{\text{eff}}}

\newcommand{\Pric} {P_{\text{r}}}
\newcommand{\hThetai} {{\hat{\Theta}}^{\text{(i)}}}
\newcommand{\hThetar} {{ \hat{\Theta}}^{\text{(r)}}}
\newcommand{\hthetar} {{ \hat{\theta}}^{\text{(r)}}}
\newcommand{\hphir} {{ \hat{\phi}}^{\text{(r)}}}
\newcommand{\Thetai} {{\Theta}^{\text{(i)}}}
\newcommand{\Thetar} {{ \Theta}^{\text{(r)}}}
\newcommand{\Thetat} {{\Theta}^{\text{t}}}
\newcommand{\Prc}{P_{r}^{metal\,can}}
\newcommand{\Prw}{P_{r}^{bottle\,water}}

\newcommand{\sreader}{s_{\text{reader}}}
\newcommand{\stag}{s_{\text{tag}}}
\newcommand{\rreader}{r_{\text{reader}}}
\newcommand{\rtag}{r_{\text{tag}}}
\newcommand{\pI}{p_{\text{I}}}
\newcommand{\pII}{p_{\text{II}}}
\newcommand{\wI}{w_{\text{I}}}
\newcommand{\wII}{w_{\text{II}}}
\newcommand{\gammaI}{\gamma_{\text{I}}}
\newcommand{\gammaII}{\gamma_{\text{II}}}
\newcommand{\Ec} {E_{\text{c}}}

\newcommand{\floor}[1] {f \left ({#1} \right )}
\newcommand{\rect}[1] {\text{Rect} \left ({#1} \right )}
\newcommand{\sinc}[1] {\text{sinc} \left ({#1} \right )}

\newcommand{\Ntag}{N_{\text{tag}}}

\newcommand{\pos} {\mathbf{p}}
\newcommand{\pes} {\mathbf{\hat{p}}}
\newcommand{\err} {e\left( \pos \right)}
\newcommand{\errx} {e_{\text{th}}}%{e^\star}

\def\dsp{\displaystyle}


\def\erfc{{\text{erfc}}}
\def\erf{{\text{erf}}}
\def\inve{{\text{inverfc}}}
\def\teq{\triangleq}
\def\bs{$\blacksquare$}
%\def\sinc{{\text{sinc}}}ì
\newcommand{\rank}[1]{{\rm rank} \left ( #1 \right )}

\newcommand{\Cfunc}[1]{{C^{(\text{#1})}}}
\newcommand{\cvect}[1]{{\mathbf{c}^{(\text{#1})}}}
\newcommand{\ucvect}[1]{{\underline{{\mathbf{c}}}^{(\text{#1})}}}
\newcommand{\epsilonvect}[1]{{\mathbf{\varepsilon}^{(\text{#1})}}}
\newcommand{\uchat}[1]{{\underline{\hat{\mathbf{c}}}^{(\text{#1})}}}
\newcommand{\chat}[1]{{\hat{\mathbf{c}}^{(\text{#1})}}}
\newcommand{\Rc}[2]{{R_c^{(\text{#1})}}{({#2})}}
\newcommand{\Rhat}[1]{{\mathbf{\hat{R}}^{(\text{#1})}}}
\newcommand{\R}[1]{{\mathbf{R}^{(\text{#1})}}}
\newcommand{\Rij}[2]{{\mathbf{R}^{(\text{#1})}_{\text{#2}}}}
\newcommand{\cij}[2]{{{c}^{(\text{#1})}_{#2}}}
\newcommand{\ccij}[2]{{{c}^{(\text{#1}) *}_{#2}}}
\newcommand{\Qtot} {Q}
\newcommand{\IK} {I_{\text{K}}}
\newcommand{\aIK} {\overline{I}_{\text{K}}}
\newcommand{\cIK} {\tilde{I}_{\text{K}}}
\newcommand{\ISK} {I_{\text{SK}}}
\newcommand{\aISK} {\overline{I}_{\text{SK}}}
\newcommand{\cISK} {\tilde{I}_{\text{SK}}}
\newcommand{\Identity}[1]{{\mathbf{I}_{#1}}}
\newcommand{\Sc}[1]{{S_{\text{c}}^{(\text{#1})}}}
\newcommand{\tSc}[2]{{\widetilde{S}_{{\text{c}}_{\text{#1}}}^{(\text{#2})}}}
\newcommand{\tS}[1]{{\mathbf{\widetilde{S}}^{(\text{#1})}}}
\newcommand{\tP}{\widetilde{P}(\tau)}
\newcommand{\ap} {{a'}}
\newcommand{\Ap} {{A'}}

\newcommand{\dEve} {d_{\text{Eve}}}
\newcommand{\NEve} {N_{\text{Eve}}}
\newcommand{\MEve} {M_{\text{Eve}}}

\newcommand{\Dset} {\mathcal{D}}
\newcommand{\GP}[1] {\mathcal{GP}\left ( #1 \right )}

\newcommand{\argmax}[1]{\underset{{#1}}{\operatorname{argmax}}}
\newcommand{\argmin}[1]{\underset{{#1}}{\operatorname{argmin}}}

%%%%%%%%% ML DERIVATIONS %%%%%%%%%

% VECTORS
\newcommand{\rvect}{{\bold{r}^{(m)}}}
\newcommand{\gvect}{{\bold{g_{l}}^{(m)}}}
\newcommand{\avect}{{\bold{a}^{(m)}}}
\newcommand{\nvect}{{\mathbf{n}^{(m)}}}
\newcommand{\svect}{{\bold{s}^{(m)}}}

\newcommand{\wvect}[1]{{\bold{w}^{(m)}_{#1}}}
\newcommand{\wvectT}[1]{{{\bold{w}^{(m)}}^{T}_{#1}}}



% MATRICES

%\newcommand{\Wm}{{\bold{W}^{(m)}_{\boldp}}}
%\newcommand{\Xm}{{{\boldsymbol{\chi}^{(m)}_{\boldp}}}}
%\newcommand{\Rm}{{\bold{R}^{(m)}_{\boldp}}}
%\newcommand{\Wm}[1]{{\bold{W}\!_{(\!m\!)}\!^{#1}({\boldp})}}
%%%%%%%%%%\newcommand{\Wm}[1]{{\bold{W}\!^{(\!m\!)}\!^{#1}({\boldp})}}
%%%%%%%%%%\newcommand{\Hm}[1]{{\bold{H}^{(\!m\!)}\!^{#1}({\boldp})}}
\newcommand{\Wm}[1]{{\bold{W}\!_{(\!m\!)}\!^{#1}({\boldp})}}
%\newcommand{\Hm}[1]{{\bold{H}_{(\!m\!)}\!^{#1}({\boldp})}}
%\newcommand{\Xim}[1]{{\boldsymbol{\Xi}^{(\!m\!)}\!^{#1}({\boldp})}}
\newcommand{\Xim}[1]{{\boldsymbol{\Xi}^{#1}}}
\newcommand{\XmTC}[1]{{{\boldsymbol{\chi}_{(\!m\!)}\!^{#1}({\boldp})}}}
\newcommand{\RmTC}[1]{{\bold{R}_{(\!m\!)}\!^{#1}({\boldp})}}
\newcommand{\Xm}[1]{{{\tilde{\boldsymbol{\chi}}_{(\!m\!)}\!^{#1}({\boldp})}}}
\newcommand{\Rm}[1]{{\tilde{\bold{R}}_{(\!m\!)}\!^{#1}({\boldp})}}

%boxes inside matrices
%\newcounter{nodecount}
%\newcommand\mn[1]{%
%\addtocounter{nodecount}{1}%
%\tikz \node (\arabic{nodecount}) {$#1$};}
%\tikzstyle{every picture}+=[remember picture,baseline]
%\tikzstyle{every node}+=[inner sep=2pt,anchor=base,align=center,text depth=.25ex,outer sep=1.5pt]
%\tikzstyle{every path}+=[thick]



% SCALARS
\newcommand{\Etx}{\breve{E}_{T}}
\newcommand{\as}[3]{a_{{#1},{#2}}^{#3}(\boldp)}
\newcommand{\ta}[1]{\tau_{{#1},{m}}(\boldp,t_0)}
\newcommand{\D}[1]{D_{{#1},m}(\boldp)}


% funzioni
\newcommand{\ONE}[2]{{\mathbbm{1}}_{#1}\left({#2}\right)}


% operazioni
\newcommand{\convZ}{*}
\newcommand{\conjZ}{^{\dag}}
\newcommand{\argmaxZ}[1]{\operatorname*{argmax}_{#1}}
\newcommand{\argminZ}[1]{\operatorname*{argmin}_{#1}}
\newcommand{\sincZ}{\text{sinc}}

% operatori, trasformate, funzioni lineari
\newcommand{\EXZ}[1] {{\mathbb{E}}\left\{{#1}\right\}}
\newcommand{\EXZBig} {\mathbb{E}}
%\newcommand{\V}[1] {\left|#1\right|}

% variabili

\newcommand{\cnZ}{\mathsf{c}}
\newcommand{\chatZ}{\hat{\mathsf{c}}}
\newcommand{\sZ}{\mathbf{x}}

\newcommand{\srZ}{\mathsf{s}}
\newcommand{\rtheta}{\mathsf{\theta}}
\newcommand{\x}{\boldsymbol{\mathsf{x}}}
\newcommand{\xvect}{\boldsymbol{\mathsf{x}}}

\newcommand{\xnk}{x_{n,k}}
\newcommand{\xkn}{x_{k,n}}
\newcommand{\xno}{x_{n,0}}
\newcommand{\xko}{x_{k,0}}
\newcommand{\hatsr}{\hat{\mathsf{s}}}

%\newcommand{\0}{\mathbf{0}}

% insiemi

\newcommand{\RZ}{\mathbb{R}^2}
%\newcommand{\C}{\mathbb{C}}

\newcommand{\Nset}{\mathcal{N}}
\newcommand{\Vset}{\mathcal{V}}

\newcommand{\rc}{r_{\text{c}}}
\newcommand{\Pe}{P_{\text{e}}}
%\newcommand{\SNR}{\mathsf{SNR}}
\newcommand{\SNR}{\text{SNR}}


\newcommand{\bX} {{\bf{X}}}
\newcommand{\bW} {{\bf{W}}}
\newcommand{\bw} {{\bf{w}}}
\newcommand{\bY} {{\bf{Y}}}

\newcommand{\Zm} {Z_{\text{m}}}
\newcommand{\zm} {z_{\text{m}}}



\newcommand{\boldtp} {{\bf{t{'}}}}
\newcommand{\boldsp} {{\bf{s{'}}}}
\newcommand{\boldrp} {{\bf{r{'}}}}
\newcommand{\boldrpp} {{\bf{r{''}}}}

\newcommand{\versorr} {\hat{\bf{r}}}
\newcommand{\versorp} {\hat{\bf{p}}}
\newcommand{\versors} {\hat{\bf{s}}}

\newcommand{\versorn} {\hat{\bf{n}}}
\newcommand{\versork} {\hat{\bf{k}}}
\newcommand{\versorki} {\hat{\bf{k}}^{\text{inc}}}
\newcommand{\versorkr} {\hat{\bf{k}}^{\text{ref}}}

\newcommand{\versorx} {{\hat{\bf{x}}}}
\newcommand{\versory} {{\hat{\bf{y}}}}
\newcommand{\versorz} {{\hat{\bf{z}}}}

\newcommand{\rxp} {{r'_x}}

\newcommand{\rx} {r_x}
\newcommand{\ry} {r_y}
\newcommand{\rz} {r_z}
\newcommand{\tx} {t_x}
\newcommand{\ty} {t_y}
\newcommand{\tz} {t_z}
\newcommand{\sx} {s_x}
\newcommand{\sy} {s_y}
\newcommand{\sz} {s_z}


\newcommand{\xo} {x_{0}}
\newcommand{\yo} {y_{0}}
\newcommand{\zo} {z_{0}}

\newcommand{\tox} {t_{0_x}}
\newcommand{\toy} {t_{0_y}}
\newcommand{\toz} {t_{0_z}}

\newcommand{\rox} {r_{0_x}}
\newcommand{\roy} {r_{0_y}}
\newcommand{\roz} {r_{0_z}}

\newcommand{\hatbx} {{\bf{\hat{x}}}}
\newcommand{\hatby} {{\bf{\hat{y}}}}
\newcommand{\hatbz} {{\bf{\hat{z}}}}
\newcommand{\hatbr} {{\bf{\hat{r}}}}
\newcommand{\hatbn} {{\bf{\hat{n}}}}


\newcommand{\Vt} {V_{\text{T}}}
\newcommand{\Vr} {V_{\text{R}}}
\newcommand{\Scal} {\mathcal{S}}
\newcommand{\Acal} {\mathcal{A}}
\newcommand{\Sr} {\mathcal{S}_{\text{R}}}
\newcommand{\St} {\mathcal{S}_{\text{T}}}
\newcommand{\Kt} {K_{\text{T}}}
\newcommand{\Kr} {K_{\text{R}}}

\newcommand{\Sx} {S_{\text{x}}}
\newcommand{\Sy} {S_{\text{y}}}
\newcommand{\Lx} {L_{\text{x}}}
\newcommand{\Ly} {L_{\text{y}}}
\newcommand{\Lz} {L_{\text{z}}}
\newcommand{\At} {A}
\newcommand{\Ar} {A_{\text{R}}}
\newcommand{\AR} {{\text{AR}}}

\newcommand{\Nr} {N_{\text{r}}}
\newcommand{\Nt} {N_{\text{t}}}
\newcommand{\Nmin} {N_{\text{min}}}
\newcommand{\Lr} {L_{\text{R}}}
\newcommand{\Lt} {L_{\text{T}}}


\newcommand{\Ptx} {P_{\text{T}}}
\newcommand{\Prx} {P_{\text{R}}}

\newcommand{\Gt} {G_t}
\newcommand{\Gr} {G_r}
\newcommand{\Gi} {G_{\text{I}}}
\newcommand{\Glis} {G_{\text{LIS}}}

\newcommand{\Gc} {G_{\text{c}}}

\newcommand{\Ge} {G_{\text{e}}}
\newcommand{\Ae} {A_{\text{e}}}
\newcommand{\Ne} {N_{\text{e}}}
\newcommand{\Nex} {N_x}
\newcommand{\Ney} {N_y}


%\newcommand{\Green} {{\bf {\cal{ G}}}}
%\newcommand{\Em} {{\bf{\it{ E}}}}
%\newcommand{\Jm} {{\bf {\cal{ J}}}}

\newcommand{\Green} {{\bf \it G} }
\newcommand{\Em} {{\bf \it E}}
\newcommand{\Hm} {{\bf \it H}}
\newcommand{\Jm} {{\bf \it J}}

\newcommand{\Jee} {{\bf \it J_{\text{e}}}}
\newcommand{\Jem} {{\bf \it J_{\text{m}}}}
\newcommand{\Js} {{\bf \it J_{\text{s}}}}
\newcommand{\Jei} {{\bf \it J^{\text{i}}_{\text{e}}}}
\newcommand{\Jmi} {{\bf \it J^{\text{i}}_{\text{m}}}}
\newcommand{\Ei} {{\bf \it E^{\text{inc}}}}
\newcommand{\Er} {{\bf \it E^{\text{ref}}}}
\newcommand{\Eim} {{  E^{\text{inc}}}}
\newcommand{\Erm} {{  E^{\text{ref}}}}
\newcommand{\Et} {{\bf \it E^{\text{t}}}}
\newcommand{\Etau} {{\bf \it E^{\tau}}}
\newcommand{\Htau} {{\bf \it H^{\tau}}}
\newcommand{\Eplus} {{\bf \it E^{\text{+}}}}
\newcommand{\Eminus} {{\bf \it E^{\text{-}}}}

\newcommand{\Hr} {{\bf \it H^{\text{ref}}}}
\newcommand{\Ht} {{\bf \it H^{\text{t}}}}
\newcommand{\Hplus} {{\bf \it H^{\text{+}}}}
\newcommand{\Hminus} {{\bf \it H^{\text{-}}}}

\newcommand{\thetai} {  \theta^{\text{(i)}}}
\newcommand{\thetar} {  \theta^{\text{(r)}}}
\newcommand{\phii} {  \phi^{\text{(i)}}}
\newcommand{\phir} {  \phi^{\text{(r)}}}


\newcommand{\um} {{\bf \it u}}
\newcommand{\vm} {{\bf \it v}}

\newcommand{\bphi} {\it \phi}
\newcommand{\bpsi} {\it  \psi}

\newcommand{\DOF} {\text{DOF}}


\newcommand{\Upx} { U_x^{+}(r_x) }
\newcommand{\Umx} { U_x^{-}(r_x) }
\newcommand{\Upy} { U_y^{+}(r_y) }
\newcommand{\Umy} { U_y^{-}(r_y) }


\newcommand{\ver}[1] {\text{ver} \left (  {#1}  \right )}

